Proximal algorithms for constrained composite optimization, with applications to solving low-rank SDPs

We study a family of (potentially non-convex) constrained optimization problems with convex composite structure. Through a novel analysis of non-smooth geometry, we show that proximal-type algorithms applied to exact penalty formulations of such problems exhibit local linear convergence under a quadratic growth condition, which the compositional structure we consider ensures. The main application of our results is to low-rank semidefinite optimization with Burer-Monteiro factorizations. We precisely identify the conditions for quadratic growth in the factorized problem via structures in the semidefinite problem, which could be of independent interest for understanding matrix factorization.

==> PaperV4_arXiv/general-invariance.tex <==
\section{Extension to general comopsite problems
  with invariance}
\label{appendix:invariance}
Our geometry and algorithmic results in Section~\ref{section:geometry}
and~\ref{section:algorithm} can hold in a setting that is more general
than the penalized SDP. However, it requires a great amount of detail
to precisely spell out this generality. In this appendix, we present a
class of constrained composite problems that contains
problem~\eqref{problem:constrained-bm} as a special case, and describe
the extension of our results into this general setting.

\subsection{Problem setup}
We consider a class of constrained composite optimization problems
with invariance, aiming to generalize the Burer-Monteiro factorization
for SDPs. Consider the problem
\begin{equation}
  \label{problem:constrained-composite}
  \begin{aligned}
    \minimize & ~~ f(c(x)) \\
    \subjectto & ~~ G(c(x)) = Ac(x) - b = 0.
  \end{aligned}
\end{equation}
In the above, $f:\R^m\to\R$ is a smooth convex function,
$c:\R^n\to\R^m$ is a smooth mapping, with properties further specified
below, $A\in\R^{k\times m}$, and $b\in\R^k$.

Problem~\eqref{problem:constrained-composite} is motivated by the
related convex problem
\begin{equation}
  \label{problem:constrained-convex}
  \begin{aligned}
    \minimize_{y\in\mc{Y}} & ~~ f(y) \\
    \subjectto & ~~ G(y) = Ay - b = 0.
  \end{aligned}
\end{equation}
In the above, $\mc{Y}\subseteq\R^m$ is a convex set that contains the
image of $c$: $c(\R^n)\subseteq\mc{Y}$. Clearly,
problem~\eqref{problem:constrained-convex} is convex and in principle
can be efficiently solved. However, there are certain scenarios where
one wish to solve~\eqref{problem:constrained-composite} instead. For
example, suppose we know (from prior knowledge) that the solution
$y_\star$ to~\eqref{problem:constrained-convex} satisfies
$y_\star=c(x_\star)$ for some $x_\star$, then $x_\star$ is the global
minimum of~\eqref{problem:constrained-composite}, so solving this
composite problem also gives the solution to the convex problem.
Furthermore, when $n\ll m$,
problem~\eqref{problem:constrained-composite} might be more amenable
to local search methods, albeit being non-convex.

An example for the pair of problems above are
problems~\eqref{problem:constrained-sdp}
(with $\mc{Y}=\symm^p$) and its Burer-Monteiro factorization
(problem~\eqref{problem:constrained-bm} with
$\R^{pr}=\vec(\R^{p\times r})$ and $c(R)=RR^\top\in\mc{Y}$).

\subsection{Assumptions}
\label{section:invariance-assumptions}
We aim to work out a set of assumptions that generate our results in
the Burer-Monteiro case as while making sense in its own. First, we
shall define invariance through $c$: we say $x_1,x_2\in\R^n$ are
equivalent if $c(x_1)=c(x_2)$. Now, define the distance w.r.t $c$ as
\begin{equation*}
  \dist_c(x_1, x_2) = \inf_{c(x_1')=c(x_1),c(x_2')=c(x_2)} \ltwo{x_1'
    - x_2'}.
\end{equation*}
Note: for this distance to make sense (so that not all distance are
zero), $c$ cannot have ``scalings'' in 
its invariance; it can only ``rotate'' things. To make this precise,
we make the following assumption. 
\begin{assumption}[Orthogonal invariance group]
  \label{assumption:orthogonal-group}
  There exists an invariance group corresponding to $c$, that is, a
  group $\Omega$ that is a subgroup of $O(n)$ satisfying
  \begin{equation*}
    c(x_1) = c(x_2) \iff x_2 = Ux_1~\text{for some}~U \in \Omega.
  \end{equation*}
\end{assumption}
We have the following result.
\begin{lemma}
  Under Assumption~\ref{assumption:orthogonal-group}, we have
  \begin{equation*}
    \dist_c(x_1,x_2) = \inf_{c(x_2')=c(x_2)} \ltwo{x_1 - x_2'} =
    \inf_{U\in\Omega} \ltwo{x_1 - Ux_2}.
  \end{equation*}
\end{lemma}

We now state our assumptions on $\vphi_f(x)=f(c(x))$ that generalize
Assumptions 1 - 3.
\begin{assumption}[Smoothness]
  \label{assumption:general-smoothness}
  The functions $f(c(\cdot))$ has Lipschitz gradients and Hessians,
  and is locally Lipschitz around $x_\star$. 
\end{assumption}
\begin{assumption}[Quadratic growth]
  \label{assumption:general-quadratic-growth}
  Problem~\eqref{problem:constrained-composite} has $\alpha$-local
  quadratic growth around a local minimum $x_\star$ if there exists
  some $\eps>0$ and $\alpha>0$ such that for any $x$ with
  $\dist_c(x,x_\star)\le \eps$, we have
  \begin{equation*}
    f(c(x)) - f(c(x_\star)) \ge \frac{\alpha}{2} \cdot \dist_c(x,x_\star)^2.
  \end{equation*}
\end{assumption}

Now we turn to the constraint qualification (CQ) condition.
\begin{assumption}[Constraint qualification]
  \label{assumption:general-constraint-qualification}
  Problem~\eqref{problem:constrained-composite} satisfies LICQ around
  $x_\star$, that is, the matrix $A\grad c(x_\star)\in\R^{k\times n}$
  has full row rank.
\end{assumption}
We claim that the above condition is well-defined, i.e. it does not
depend on the choice of the minimum $x_\star$. Indeed, picking an
equivalent minimum $x_\star'$, then there exists some $U\in\Omega$
such that $x_\star'=Ux_\star$. As $c(Ux)=c(x)$ for all $x$, taking the
Jacobian on both sides gives
\begin{equation*}
  \grad c(x) = \grad c(Ux) U^\top.
\end{equation*}
Thus, $A\grad c(x_\star') = A\grad c(Ux_\star) = A\grad c(x_\star)
U$, and so the row rank of $A\grad c(x_\star')$ and $A\grad
c(x_\star)$ must be the same.

\subsection{Results}
Under the above assumptions, our main geometry and algorithm result
(Theorem~\ref{theorem:quadratic-implies-regularity}
and~\ref{theorem:linear-convergence}) hold in this more general
setting. We present their counterparts here, and the proofs are
completely parallel to the presented proofs on matrix problems. Let
\begin{equation}
  \label{problem:penalized-general}
  \vphi(x) = f(c(x)) + \lambda\ltwo{Ac(x)-b}
\end{equation}
denote the penalized objective.

\begin{theorem}
  Under Assumptions~\ref{assumption:orthogonal-group},~
  \ref{assumption:general-smoothness},~
  \ref{assumption:general-quadratic-growth},
  and~\ref{assumption:general-constraint-qualification}, 
  there exists constants $\ell\le 5$, $\Lambda>0$, and a neighborhood
  $\mc{X}$ of the minimizing set in which setting the penalty
  parameter $\lambda\ge \Lambda$, $\vphi$ satisfies norm convexity
  with parameter $\ell$ and sub-differential regularity with constant
  $4\ell/\alpha$. 
\end{theorem}
\begin{theorem}
  Under Assumptions~\ref{assumption:orthogonal-group},~
  \ref{assumption:general-smoothness},~
  \ref{assumption:general-quadratic-growth},
  and~\ref{assumption:general-constraint-qualification}, and let the
  conditions of Theorem~\ref{theorem:linear-convergence} hold
  with the problem replaced with
  minimizing~\eqref{problem:penalized-general}. Then the prox-linear
  method has local linear convergence.
\end{theorem}

==> PaperV4_arXiv/initialization.tex <==
\section{Storage-optimal initialization}
The convergence guarantee in
Corollary~\ref{corollary:sdp-linear-convergence} is local -- it
requires an initializer $R^0$ near the minimizing set $S$. In this
section, we briefly describe how to obtain such an initialization in
practice for an interesting sub-class of problems of the
form~\eqref{problem:constrained-sdp}. Recall that we require a point
$R$ with $\dist(R,S)$ small
-- under linear or quadratic growth, this is roughly equivalent to
requiring $\vphi(R)-\vphi^\star$ small.

\paragraph{Sketchy Frank-Wolfe method} To achieve this, we solve the
original convex formulation~\eqref{problem:constrained-sdp} to get a
point $X\succeq 0$ that has low optimality gap and low feasibility
gap. Further, we would like that our algorithm only stores $O(nr)$
variables, as is required in large-scale applications.

We extend the idea of sketchy Frank-Wolfe
methods~\cite{YurtseverUdTrCe17} onto constrained problems. More
precisely, suppose $f(X)$ depdens only on a low-dimensional linear
function of $X$: for some $\mc{C}:\symm^n\to\R^d$,
\begin{equation*}
  f(X) = f(\mc{C}(X)).
\end{equation*}
We form the augmented Lagrangian for
problem~\eqref{problem:constrained-sdp}:
\begin{equation*}
  L_\rho(X,\lambda) = f(\mc{C}(X)) + \<\lambda,\mc{A}(X)-b\> +
  \frac{\rho}{2}\ltwo{\mc{A}(X)-b}^2.
\end{equation*}
Starting from $X^0,\lambda^0$ and fixed $\rho$, we run the
method of multipliers updates:
\begin{equation}
  \label{equation:method-of-multipliers}
  X^{k+1} = \argmin_{X} L_\rho(X,\lambda^k),~~~\lambda^{k+1} =
  \lambda^k + \rho(\mc{A}(X^{k+1})-b).
\end{equation}
Each round requires solving a smooth convex problem, in which we use
the Frank-Wolfe method: we figure out an upper bound $\alpha\ge
\tr(X^\star)$, and run Frank-Wolfe methods on the problem
\begin{align*}
  \minimize & ~~ L_\rho(X,\lambda^k) \\
  \subjectto & ~~ X \succeq 0,~~\tr(X) \le \alpha,
\end{align*}
which iteratively updates
\begin{equation}
  \label{equation:frank-wolfe}
  S^{j+1} = \argmin_{X\ge 0,\tr(X)\le\alpha}\<\grad
  L_\rho(X^j,\lambda), X\>,~~~X^{j+1} = (1-\tau_{j+1})X^j +
  \tau_{j+1}S^{j+1} 
\end{equation}
with $\tau_j=2/(j+2)$.
The first part has an explicit solution: letting $v=v_{\min}(\grad
L_\rho(X^j,\lambda))$, we have
\begin{equation}
  \label{equation:fw-eigenvector}
  S^{j+1} = \left\{
    \begin{aligned}
      \alpha \cdot vv^\top,~~\lambda_{\min}(\grad L_\rho(X^j,\lambda))
      < 0 \\
      0,~~\lambda_{\min}(\grad L_\rho(X^j,\lambda)) \ge 0.
    \end{aligned}
  \right.
\end{equation}
As the updates $S^j$ are at most rank-one, and the solution $X^\star$
also has low rank, we only maintain the linear maps $\mc{A}(X)$,
$\mc{C}(X)$ necessary for solving the problem, and a rank $O(r)$
sketch of $X$ throughout executions of the Frank-Wolfe method. We
repeat the method of multipliers
update~\eqref{equation:method-of-multipliers} with a few Frank-Wolfe
iterations in each inner minimization problem.

It can be shown that
with properly chosen inner iteration numbers, the optimality gap
$f(X^k)-f^\star$ and feasibility gap $\ltwo{\mc{A}(X^k)-b}$ converge
to zero with explicitly characterized rates~\cite{LanMo16}. Hence by
continuity and uniqueness of the solution, $X^k\to
X^\star$ in the limit. In particular, as $X^\star$ has rank $r$, the
matrices $X^k$ will be approximately rank $r$ for large $k$, and their
best rank $r$ approximations will also converge to $X^\star$. We do
not have a bound for the number of iterations to reach
$\lfro{X^k-X^\star}\le\eps$, but note under the assumption that
problem~\eqref{problem:constrained-sdp} have quadratic growth over all
$X\succeq 0$ (stronger than
Assumption~\ref{assumption:quadratic-growth}), then it is
straightforward to get a convergence rate and complexity bound. 

After some termination criterion is
satisfied, we reconstruct a rank-$r$ approximation $RR^\top$ to the
current iterate $X^k$. It is guaranteed that $\lfro{RR^\top-X^k} \le
O(\sigma_{r+1}(X^k))$ with high
probability~\cite{YurtseverUdTrCe17}. For sufficiently large $k$,
$X^k$ will be close to $X^\star$ with small $\sigma_{r+1}(X^k)$, giving
an initialization $R$ close to the minimizing set.

% \paragraph{Stability} To guarantee that the above algorithm does give
% a close initialization, we
% need to argue that a point with low optimality gap and low feasibility
% gap is close to the solution $X^\star$. Fortunately, we could use
% linear or quadratic growth of
% $\vphi(R)=f(RR^\top)+\lambda\ltwo{\mc{A}(RR^\top)-b}$ to argue that
% this is indeed true. We will not go into details of such stability
% arguments.

==> PaperV4_arXiv/optimality.tex <==
\section{Global optimality in the penalized objective}
\label{section:optimality}
We begin by showing when $\lambda>\ltwo{y}$, the exact penalty method
preserves the minimizing set, so that
problems~\eqref{problem:constrained-bm}
and~\eqref{problem:penalized-bm} have the same set of global
minima. Results of this type are classical in the non-linear
programming literature; see \cite[Theorem~3.3]{Han77} for example.

Let $g(X)=\ltwo{\mc{A}(X)-b}$ be the penalty term and
\begin{equation*}
  h_\lambda(X) \defeq f(X) + \lambda g(X) = f(X) +
  \lambda\ltwo{\mc{A}(X)-b}
\end{equation*}
be the penalized objective. We will often omit the subscript $\lambda$
when it is clear from the context. Define the factorization map
$c:\R^{n\times r}\to\mc{S}^n$ as 
\begin{equation*}
  c(R) = RR^\top,
\end{equation*}
the factorized objective can be written as $\vphi(R) = h_\lambda(c(R))
= \vphi_f(R) + \lambda\vphi_g(R)$, where
\begin{equation*}
  \vphi_f(R) \defeq f(c(R))=f(RR^\top),~~\vphi_g(R) \defeq g(c(R)) =
  \ltwo{\mc{A}(RR^\top)-b}.
\end{equation*}
The function $\vphi(\cdot)=h(c(\cdot))$ has a convex-composite
structure: it is the composition of of a smooth mapping and a convex
function. However, such functions are non-convex and non-smooth in
general. Further, unlike in smooth cases where one can often find a
locally convex region near the local minimum, here even near $R_\star$
the objective is still non-convex and non-smooth.

\subsection{Optimality in the PSD space}
Let $X_\star$ be the solution to the original semidefinite
program~\eqref{problem:constrained-sdp}. Throughout the paper we
assume that the solution is unique. By convexity and strong
duality, $X_\star$ satisfies the first-order optimality condition:
there exists an optimal dual variable $y_\star\in\R^m$ such that
\begin{equation*}
  \grad f(X_\star) + \mc{A}^*(y_\star) \in -\mc{N}_\psd(X_\star).
\end{equation*}
In other words, $(X_\star, y_\star)$ forms a min-max optimum of the
Lagrangian
\begin{equation*}
  L(X, y) = f(X) + \<y, \mc{A}(X)-b\>.
\end{equation*}
Throughout this paper we assume that $y_\star\neq 0$; otherwise the
constraints do not affect the problem.

As $X_\star$ minimizes $L(X,y_\star)$ for $X\succeq
0$. A simple consequence of strong duality is
that $X_\star$ is the only global minimum of $h_\lambda$ for
$\lambda\ge \ltwo{y_\star}$. 
\begin{lemma}
  \label{lemma:penalized-global-min}
  We have
  \begin{equation*}
    h(X) \ge L(X, y_\star) + (\lambda -
    \ltwo{y_\star})\ltwo{\mc{A}(X)-b}.
  \end{equation*}
  In particular, when $\lambda\ge\ltwo{y_\star}$, $X_\star$ is a
  global minimum of $h_\lambda$; when $\lambda>\ltwo{y_\star}$,
  $X_\star$ is the unique global minimum.
\end{lemma}
The proof is in Appendix~\ref{appendix:proof-optimality}.

\subsection{Optimality in the factorized space}
An immediate corollary of Lemma~\ref{lemma:penalized-global-min} is
that $R_\star$ is also a global minimum of $\vphi(R)=h(RR^\top)$ when
$\lambda\ge \ltwo{y_\star}$.
Note that, however, $R_\star$ is not the unique global minimum: for
any orthogonal matrix $Q\in\R^{r\times r}$, we have that $R_\star
R_\star^\top=(R_\star Q)(R_\star Q)^\top$, so $R_\star Q$ is also a
global minimum. Let $S\subset\R^{n\times r}$ denote the minimizing set
of $\vphi(R)$ and
\begin{equation*}
  S_\star \defeq \set{R_\star Q: Q^\top Q=QQ^\top=I_{r\times r}} =
  \set{R: RR^\top=X_\star}
\end{equation*}
denote the set of equivalent factorizations, then $S_\star\subseteq
S$. We summarize these observations into the following corollary.
\begin{corollary}
  We have $S_\star\subseteq S$ if $\lambda\ge\ltwo{y_\star}$ and
  $S_\star=S$ if $\lambda>\ltwo{y_\star}$.
\end{corollary}
Consequently, as long as we choose $\lambda>\ltwo{y_\star}$, the only
global minima are those $R$ such that
$RR^\top=R^{\star}R_\star^\top=X_\star$, guaranteeing that the
penalized objective has no spurious global minimum. In the following,
we will assume that $\lambda>\ltwo{y_\star}$ and thus $S=S_\star$.

\subsection{The Procrustes problem}
To better understand the factorization map $X=RR^\top$, we provide
some background on the Procrustes problem, based on
\citet{TuBoSiSoRe16}. In particular, we obtain an geometric
characterization of the distance $\dist(R,S)$.

Let $R \in \R^{n
  \times r}$ and $Q \in \R^{n \times r}$ be arbitrary matrices, $n \ge
r$. The Procrustes problem is the alignment problem
\begin{equation*}
  \minimize_{\Omega \in \R^{r \times r}, \Omega^T \Omega = I_r}
  \lfro{R - Q\Omega}^2.
\end{equation*}
By expanding the Frobenius norm, this is equivalent to maximizing $\<R,
Q\Omega\> = \tr(R^TQ \Omega)$ over orthogonal matrices
$\Omega$. Writing the singular value decomposition of $R^T Q = U
\Sigma V^T$, where $U, V \in \R^{r \times r}$ are orthogonal and
$\Sigma \in \diag(\R_+^r)$, we see
\begin{equation*}
  \tr(R^T Q \Omega)
  = \tr(\Sigma V^T \Omega U)
  \le \tr(\Sigma),
\end{equation*}
where we have used von-Neumann's trace inequality, with equality
achieved by $\Omega = V U^T$.
If we define the difference $\Delta = R - Q\Omega$, then we have
\begin{equation*}
  R^T Q \Omega
  = U \Sigma V^T V U^T = U \Sigma U^T
  = U V^T V \Sigma U^T = \Omega^T Q^T R \succeq 0
\end{equation*}
and that
$\Delta^T Q \Omega = (Q \Omega)^T \Delta$ is symmetric. As a direct
consequence, we have
\begin{equation*}
  \dist(R,S) = \min_{\Omega\in\R^{r\times
      r},\Omega^\top\Omega=I_{r\times r}} \lfro{R-R_\star\Omega}^2
\end{equation*}
equals the optimal value of the Procrustes problem.
We say that $R$ and $R_\star\in S$ are optimally aligned if
$\lfro{R-R_\star}=\dist(R,S)$, i.e. when the minimizing $\Omega$ is
the identity.

The factorization $X=RR^\top$ brings in a great deal of non-uniqueness
issues, but as we will see, this creates no additional challenge for
our developments. To name one, when we talk about neighborhoods of
$S$, the neighborhood can always be taken as
$\bigcup_{R_\star\in S}\ball_2(R_\star,\eps)$ for some $\eps$. To see
this, we can first perform our analysis $\ball_2(R_\star,\eps)$ for
one $R_\star$, then by the invariance under the transform
$R\mapsto R\Omega$, the property will also hold in
$\ball_2(R_\star\Omega,\eps)$ for all orthogonal matrix $\Omega$.


==> PaperV4_arXiv/over-specification.tex <==
\section{The effect of rank over-specification}
\label{section:over-specification}
A drawback of our factorization approach is that we require knowing
$r={\rm rank}(X^\star)$ before even obtaining the solution. In many real
problems, the true rank $r$ cannot be known exactly -- we only know an
upper bound on the rank. In these cases, a common strategy is to choose
an upper bound $k$ on the rank and factorize $X=UU^\top$ for
$U\in\R^{n\times k}$. It has been frequently observed that a moderate
over-specification of the rank will not slow down convergence.

In this section, we explain this phenomena via a careful analysis on
the rank over-specified version of
problems~\eqref{problem:constrained-bm}
and~\eqref{problem:penalized-bm}. We show that over-specifying the
rank will preserve quadratic growth when $f$ is linear. In
constrast, quadratic growth will not be preserved with generic convex
$f$. 

\subsection{Generic objectives}
Our geometric result does not immediately apply to the over-specified
case. To see this, recall that we began our analysis by converting
quadratic growth of $f$ into that of $\vphi_f$
(Lemma~\ref{lemma:factorized-quadratic-growth}), whose proof relies on
Lemma~\ref{lemma:matrix-factorization-bound}, which
says that $\lfro{RR^\top-R^\star R^{\star\top}}$ grows at least
linearly in $\lfro{R-R^\star}$:
\begin{equation*}
  \lfro{RR^\top-R^\star R^{\star\top}} \ge
  \sqrt{2(\sqrt{2}-1)} \sigma_r(R^\star) \cdot \lfro{R-R^\star}.
\end{equation*}
This bound requires $\sigma_r(R^\star)>0$, or that we have
specified the correct rank $r$. If we used an upper bound $k>r$
and factorized $X^\star=U^\star U^{\star\top}$ for
$U^\star\in\R^{n\times k}$, then $\sigma_k(U^\star)=0$, and the
inequality does not say anything. The following example demonstrates
that the growth can indeed be slower when we over-specify the rank.

\begin{example}
  \label{example:overspecified-rank}
  Let $R^\star\in\R^{n\times r}$ have full column rank and
  $U^\star=[R^\star,\zeros_n]\in\R^{n\times(r+1)}$, so that $U^\star
  U^{\star\top} = X^\star$. Let $U=[R^\star,y]\in\R^{n\times(r+1)}$,
  where $y\in\R^n$ is such that $R^{\star\top}y = \zeros$. Then,
  \begin{equation*}
    U^\top U^\star = \begin{bmatrix}
      R^{\star\top}R^\star & \zeros_r \\
      y^\top R^\star & 0
    \end{bmatrix} = \begin{bmatrix}
      R^{\star\top}R^\star & \zeros_r \\
      \zeros_r^\top & 0
    \end{bmatrix} \succeq 0,
  \end{equation*}
  so $U$ and $U^\star$ are optimally aligned. However, we
  have
  \begin{equation*}
    \lfro{UU^\top - U^\star U^{\star\top}} =
    \lfro{R^\star R^{\star\top} + yy^\top - R^\star R^{\star\top}} =
    \ltwo{y}^2
  \end{equation*}
  and
  \begin{equation*}
    \lfro{U - U^\star} = \lfro{[R^\star,y] -
      [R^\star,\zeros_n]} = \ltwo{y}.
  \end{equation*}
  The distance in the PSD space depends quadratically in the distance
  in the low-rank space, not linearly. Taking
  $h(X)=\frac{1}{2}\lfro{X-X^\star}^2$ for example, the factorized
  version $\vphi(U)=h(UU^\top)$ will only have fourth-order growth
  around $U^\star$ in certain directions.
\end{example}

Knowing that $\lfro{UU^\top-U^\star U^{\star\top}}$ can be as low as
$\dist(U,U^\star)^2$, we extend
Lemma~\ref{lemma:matrix-factorization-bound} in the 
following result, showing that a quadratic lower bound is indeed
true. Consequently, any problem~\eqref{problem:constrained-sdp} with
quadratic growth will have at least fourth-order growth under
rank over-specification. 
\begin{lemma}
  \label{lemma:overspecified-factorization-bound}
  Let $U^\star,U\in\R^{n\times k}$ be such that
  $U^\top U^\star\succeq 0$, and $\Delta=U-U^\star$. Then
  \begin{equation*}
    \lfro{UU^\top - U^\star U^{\star\top}}^2 \ge
    2(\sqrt{2}-1)\max\set{\lfro{U^\star\Delta^\top},
      \frac{1}{3}\lfro{\Delta\Delta^\top}}^2 \ge
    \frac{2(\sqrt{2}-1)}{9k}\lfro{\Delta}^4.
  \end{equation*}
\end{lemma}
The proof is in
Appendix~\ref{appendix:proof-overspecified-factorization}. 

\subsection{Linear objectives}
The situation gets significantly better when our objective is
linear. We show that for linear objectives, rank
over-specification preserves quadratic growth under some mild
additional assumptions. Letting $f(X)=\<C,X\>$ for $C\in\symm^n$,
problem~\eqref{problem:constrained-sdp} reads
\begin{equation}
  \label{problem:sdp}
  \begin{aligned}
    \minimize & ~~ \<C,X\> \\
    \subjectto & ~~ \mc{A}(X) = b \\
    & ~~ X \succeq 0.
  \end{aligned}
\end{equation}
Problem~\eqref{problem:sdp} admits a rank-$r$ solution
$X^\star=R^\star R^{\star\top}$, where $R^{\star}\in\R^{n\times r}$
has full column rank and $\frac{r(r+1)}{2}\le
m$~\cite{BurerMo03,Pataki98}. Let $X^\star=Q_1\Sigma_x Q_1^\top$ be
the eigenvalue decomposition, where $Q_1\in\R^{n\times r}$ and
$\Sigma_x\in\R^{r\times r}$ is diagonal. We can then take
$R^\star=Q_1\sqrt{\Sigma_x}$. Let $Q_2\in\R^{n\times(n-r)}$ be the
orthogonal complement of $Q_1$, i.e. such that $[Q_1,
Q_2]\in\R^{n\times n}$ is an orthogonal matrix.

Let $(y,Z)\in\R^m\times \symm^n$ be dual optimal satisfying the
strict complementarity condition:
\begin{enumerate}[(1)]
\item (Dual feasibility) $Z=\mc{A}^*(y)+C\succeq 0$.
\item (Complementary slackness) $\<Z,X^\star\>=0$.
\item (Strict complementarity) $\rank(Z)=n-r$.
\end{enumerate}
It is known that under the above conditions, $X^\star$ is the unique
solution if and only if the \emph{dual non-degeneracy} conditions
hold~\cite{AlizadehHaOv97}, i.e.
\begin{quote}
  \centering
  $\set{Q_1^\top A_1Q_1,\dots,Q_1^\top A_mQ_1}$ spans $\symm^r$.
\end{quote}
We will assume a quantitative version of strict complementarity and
dual non-degeneracy.
\begin{assumption}[Strict complementarity and dual non-degeneracy]
  \label{assumption:dn}
  There exists a pair of dual optimal $(y,Z)$ such that the $(r+1)$-th
  smallest singular value is lower bounded by $\lambda>0$. There
  exists some constant $\sigmadn>0$ such that
  \begin{equation*}
    \sum_{i\in[m]} \<Q_1^\top A_iQ_1, W\>^2 \ge \sigmadn \cdot
    \lfro{W}^2,~\text{for all}~W\in\symm^r.
  \end{equation*}
\end{assumption}
Assuming this condition, we can lower bound the growth of $f$ as
follows. For any $X\succeq 0$, $\mc{A}(X)=b$, we have
$\<\mc{A}^*(y),X-X^\star\>=\<y,\mc{A}(X)-\mc{A}(X^\star)\>=0$. Hence
\begin{equation}
  \label{equation:linear-growth}
  \<C,X-X^\star\> = \<\mc{A}^*(y)+C,X-X^\star\> = \<Z,X-X^\star\> =
  \<Z,X\> \ge \lambda\lnuc{Q_2^\top XQ_2}.
\end{equation}
Unfortunately, the RHS cannot be lower bounded by $\lfro{X-X^\star}$,
so problem~\eqref{problem:sdp} will not have linear growth in
general. The following result demonstrates that the
term~$\lnuc{Q_2^\top XQ_2}$ will have quadratic growth in
$U$. See Appendix~\ref{appendix:proof-linear-overspecified} for the
proof.
\begin{lemma}
  \label{lemma:overspecified-growth}
  Let $k\ge r$, $X^\star=U^\star U^{\star\top}$ and $X=UU^\top$ for
  $U,U^\star\in\R^{n\times k}$.
  Suppose Assumption~\ref{assumption:dn} holds, and the feasible set
  \begin{equation*}
    \mc{M}_k \defeq \set{U\in\R^{n\times k}:\mc{A}(UU^\top)=b}
  \end{equation*}
  is a smooth manifold,
  then there exists a neighborhood of $U^\star$ and a positive
  constant $c>0$ such that for all feasible $X=UU^\top$ in this
  neighborhood, 
  \begin{equation*}
    \lnuc{Q_2^\top XQ_2} \ge c \cdot \dist(U,U^\star)^2.
  \end{equation*}
  The constant $c$ is
  \begin{equation*}
    c = \frac{1}{2(\kappa+1)},~~~ \kappa \defeq
    \frac{\lambda_1(X^\star)}{\lambda_r(X^\star)} \cdot 
    \frac{\sum_{i=1}^m \lfro{Q_2^\top A_iQ_1}^2}{\sigmadn}.
  \end{equation*}
\end{lemma}
Lemma~\ref{lemma:overspecified-growth} combined with the growth
bound~\eqref{equation:linear-growth} characterizes the geometry of
$\vphi_f(U)=\<C,UU^\top\>$: for $U$ feasible near the minimizing set,
we have
\begin{equation*}
  \<C,UU^\top-U^\star U^{\star\top}\> \ge \lambda\lfro{Q_2^\top
    UU^\top Q_2} \ge c\lambda \cdot \dist(U,U^\star)^2,
\end{equation*}
thus $\vphi_f$ will have quadratic growth with constant
$2c\lambda$. Consequently,
Lemma~\ref{lemma:penalized-quadratic-growth} 
extends to this case, and our main geometric result will follow by
replicating the proof of
theorem~\ref{theorem:quadratic-implies-regularity}. We summarize this
in the following theorem.
\begin{theorem}[Geometry of linear objectives under rank
  over-specification]
  \label{theorem:linear-objective-over-specified}
  Suppose $f(X)=\<C,X\>$ and
  Assumptions~\ref{assumption:constraint-non-degeneracy}
  and~\ref{assumption:dn} hold for rank $k$, then the solution to
  problem~\eqref{problem:sdp} is unique, and
  $\vphi_f(U)=\<C,UU^\top\>$ has local quadratic growth: for all $U$
  near $U^\star$ and feasible,
  \begin{equation*}
    \vphi_f(U) - \vphi_f(U^\star) \ge \frac{\alpha_{\vphi_f}}{2}
    \cdot \dist(U,U^\star)^2,
  \end{equation*}
  where $\alpha_{\vphi_f}>0$ depends on
  $(X^\star,\mc{A},\lambda,\sigmadn)$ but not $k$. Further, (noting that
  Assumption~\ref{assumption:smoothness} always holds),
  $\vphi(U)=\vphi_f(U) + \lambda \vphi_g(U)$ satisfies the norm
  convexity~\eqref{equation:comparison} and sub-differential
  regularity~\eqref{equation:regularity} (with $R$ replaced by $U$).
\end{theorem}
Theorem~\ref{theorem:linear-objective-over-specified} applies
generally to the constrained formulation of the factorized problem, 
and tells the reason why over-specifying the rank often works in
practice -- quadratic growth is carried to
problem~\eqref{problem:constrained-bm}. 

==> PaperV4_arXiv/proof-optimality.tex <==
\section{Proof of Lemma~\ref{lemma:penalized-global-min}}
\label{appendix:proof-optimality}
We have
\begin{align*}
  & \quad h_\lambda(X) = f(X) + \lambda\ltwo{\mc{A}(X)-b} = f(X) + 
    \ltwo{y_\star}\norm{\mc{A}(X)-b} +
    (\lambda-\ltwo{y_\star})\norm{\mc{A}(X)-b} \\
  & \ge f(X) + \<y_\star,\mc{A}(X)-b\> +
    (\lambda-\ltwo{y_\star})\norm{\mc{A}(X)-b} = L(X, y_\star) +
    (\lambda-\ltwo{y_\star})\norm{\mc{A}(X)-b}.
\end{align*}
In particular, when $\lambda\ge\ltwo{y_\star}$, the above
shows that for all $X\succeq 0$,
\begin{equation*}
  h_\lambda(X) \ge L(X, y_\star) \ge L(X_\star, y_\star) =
  f(X_\star) = h_\lambda(X_\star),
\end{equation*}
so $X_\star$ is a global minimum. Now, suppose
$\lambda>\ltwo{y_\star}$ and there is some $X$ such that
$h_\lambda(X)=h_\lambda(X_\star)$. From the preceding display, we
get
\begin{equation*}
  h_\lambda(X_\star) = h_\lambda(X) \ge L(X,y_\star) +
  (\lambda-\ltwo{y_\star})\ltwo{\mc{A}(X)-b} \ge  L(X_\star,y_\star)
  = h_\lambda(X_\star).
\end{equation*}
As equality holds, we must have $\mc{A}(X)=b$ and so $X$ is
feasible. Combined with $L(X,y_\star)=L(X_\star,y_\star)$, we get
$X=X_\star$, as the solution to~\eqref{problem:constrained-sdp} is
unique.
